Constraint Back-translation Improves Complex Instruction Following of Large Language Models

Large language models (LLMs) struggle to follow instructions with complex constraints in format, length, etc. Following the conventional instruction-tuning practice, previous works conduct post-training on complex instruction-response pairs generated by feeding complex instructions to advanced LLMs. However, even advanced LLMs cannot follow complex instructions well, thus limiting the quality of generated data. In this work, we find that existing datasets inherently contain implicit complex constraints and propose a novel data generation technique, constraint back-translation. Specifically, we take the high-quality instruction-response pairs in existing datasets and only adopt advanced LLMs to add complex constraints already met by the responses to the instructions, which naturally reduces costs and data noise. In the experiments, we adopt Llama3-70B-Instruct to back-translate constraints and create a high-quality complex instruction-response dataset, named CRAB. We present that post-training on CRAB improves multiple backbone LLMs' complex instruction-following ability, evaluated on extensive instruction-following benchmarks. We further find that constraint back-translation also serves as a useful auxiliary training objective in post-training. Our code, data, and models will be released to facilitate future research.

==> latex/02.pilot.tex <==
% \section{Pilot Experiments}

% \begin{figure}[t]
%     % \centering
%     \includegraphics[width=1.0\linewidth]{latex/figs/pilot.pdf} %pdf
%     \caption{Pilot experiment
%     }
%     \label{fig:Dpo_data_size}
% \end{figure}


% In evaluating the output quality of LLMs on multi-constraint complex tasks, the common focus is whether the output meets all specified constraints~\citep{sun2024conifer,he2024complex}. However, a key question remains unexplored: Do overabundance constraints in instruction affect the overall content quality of the generated output?

% To explore this question, we sampled $100$ instruction pairs from FollowBench~\citep{jiang-etal-2024-followbench} and IFEval~\citep{zhou2023instruction}, with each pair consisting of a sample instruction and its corresponding multi-constraint complex version (with over $3$ constraints). Since IFEval does not provide sample instructions, we randomly selected $50$ complex instructions and manually removed the constraints. For FollowBench, we selected level $0$ instructions along with their corresponding level $5$ counterparts. To ensure a fair comparison, we only retained instruction pairs where the core meaning of the instruction pairs remained consistent, such that the output generated from the complex instructions would still satisfy the simple versions.
% %这里的无约束/简单该如何准确的定义，虽然称作无约束，但是instruction本身就带有situation，不可能完全无约束。



